Spontaneous Breaking of Space-Time Symmetries

Kinematical and dynamical mechanisms leading to the spontaneous breaking of space-time symmetries are described. The symmetries affected are space and time translations, space rotations, scale and conformal transformations. Applications are made to solidification, string theory compactifications, the analysis of stable theories with no ground states, supersymmetry breaking and the determination of the value of the vacuum energy.

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% "physics"
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%

%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
% Non-BibTeX users please use
\begin{thebibliography}{99.}
%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references
%
% Monographs
\bibitem{monograph} H. Ibach, H. L\"uth: \textit{Solid-State
Physics}, 2nd edn (Springer, Berlin Heidelberg New York 1996) pp 45--56

% Contributed Works
\bibitem{contribution} D.M. MacKay: Visual stability and voluntary eye
movements. In: \textit{Handbook of Sensory Physiology}, vol 3, ed by R.
Jung, D.M. MacKay (Springer, Berlin Heidelberg New York 1973) pp
307--331

% Journal
\bibitem{journal} S. Preuss, A. Demchuk Jr, M. Stuke et al: Appl. Phys.
A \textbf{61}, 33 (1995)

% Theses
\bibitem{thesis} D.W.  Ross: Lysosomes and storage diseases. MA
Thesis, Columbia University, New York (1977)

\end{thebibliography}


==> svind.ist.tex <==
 delim_0 "\\idxquad "
delim_1 "\\idxquad "
delim_2 "\\idxquad "
delim_n ",\\,"
